Evaluating the Stability of Semantic Concept Representations in CNNs for Robust Explainability

Analysis of how semantic concepts are represented within Convolutional Neural Networks (CNNs) is a widely used approach in Explainable Artificial Intelligence (XAI) for interpreting CNNs. A motivation is the need for transparency in safety-critical AI-based systems, as mandated in various domains like automated driving. However, to use the concept representations for safety-relevant purposes, like inspection or error retrieval, these must be of high quality and, in particular, stable. This paper focuses on two stability goals when working with concept representations in computer vision CNNs: stability of concept retrieval and of concept attribution. The guiding use-case is a post-hoc explainability framework for object detection (OD) CNNs, towards which existing concept analysis (CA) methods are successfully adapted. To address concept retrieval stability, we propose a novel metric that considers both concept separation and consistency, and is agnostic to layer and concept representation dimensionality. We then investigate impacts of concept abstraction level, number of concept training samples, CNN size, and concept representation dimensionality on stability. For concept attribution stability we explore the effect of gradient instability on gradient-based explainability methods. The results on various CNNs for classification and object detection yield the main findings that (1) the stability of concept retrieval can be enhanced through dimensionality reduction via data aggregation, and (2) in shallow layers where gradient instability is more pronounced, gradient smoothing techniques are advised. Finally, our approach provides valuable insights into selecting the appropriate layer and concept representation dimensionality, paving the way towards CA in safety-critical XAI applications.

==> graphics/tables/grad_stab_en1d_1d.tex <==
%table
\begin{table}

\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.95}
\centering
\caption{Gradient stability in layers of EfficientNet for 1D-CAV.
%Thereby, $l_1$ is features.1.0.block.2.0, $l_2$ is features.2.0.block.3.0, $l_3$ is features.3.0.block.3.0, $l_4$ is features.4.0.block.3.0, $l_5$ is features.5.0.block.3.0, $l_6$ is features.6.0.block.3.0, $l_7$ is features.7.0.block.3.0.
}
\label{tab:grad-stability-en1d-1d}

%tabular
\begin{tabular}{c|ccccccc}

%header
\hline
\multicolumn{1}{l|}{Measure} & $l_1$ & $l_2$ & $l_3$ & $l_4$ & $l_5$ & $l_6$ & $l_7$ \\

%values
\hline
$TP$ & 492 & 469 & 499 & 514 & 527 & 410 & 279 \\
$TN$ & 475 & 459 & 475 & 456 & 450 & 566 & 720 \\
\hline
$FP$ & 13 & 35 & 16 & 16 & 14 & 12 & 0 \\
$FN$ & 20 & 37 & 10 & 14 & 9 & 12 & 1 \\
\hline
$Acc$ & 0.97 & 0.93 & 0.97 & 0.97 & 0.98 & 0.98 & 1.00 \\
\hline
$CAD, \%$ & 13.5 & 21.7 & 10.8 & 10.9 & 8.9 & 8.8 & 1.1 \\

\hline
\end{tabular}
\end{table}


==> graphics/tables/grad_stab_en3d_3d.tex <==
%table
\begin{table}

\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.95}
\centering
\caption{Gradient stability in layers of EfficientNet for 3D-CAV.
%Thereby, $l_1$ is features.1.0.block.2.0, $l_2$ is features.2.0.block.3.0, $l_3$ is features.3.0.block.3.0, $l_4$ is features.4.0.block.3.0, $l_5$ is features.5.0.block.3.0, $l_6$ is features.6.0.block.3.0, $l_7$ is features.7.0.block.3.0.
}
\label{tab:grad-stability-en3d-3d}

%tabular
\begin{tabular}{c|ccccccc}

%header
\hline
\multicolumn{1}{l|}{Measure} & $l_1$ & $l_2$ & $l_3$ & $l_4$ & $l_5$ & $l_6$ & $l_7$ \\

%values
\hline
$TP$ & 466 & 507 & 477 & 530 & 511 & 416 & 398 \\
$TN$ & 481 & 442 & 498 & 443 & 466 & 562 & 599 \\
\hline
$FP$ & 31 & 26 & 12 & 16 & 11 & 10 & 2 \\
$FN$ & 22 & 25 & 13 & 11 & 12 & 12 & 1 \\
\hline
$Acc$ & 0.95 & 0.95 & 0.97 & 0.97 & 0.98 & 0.98 & 1.00 \\
\hline
$CAD, \%$ & 13.0 & 20.3 & 10.7 & 10.0 & 9.4 & 8.3 & 1.3 \\

\hline
\end{tabular}
\end{table}

